Artin Presentations of the Trivial Group and Hyperbolic Closed Pure $3$-Braids

We consider a special class of framed links that arise from the hexatangle. Such links are introduced in [arXiv:0807.1677], which was also analyzed when the 3-manifold obtained after performing integral Dehn surgery on closed pure 3-braids is $S^3$. In the present paper, we analyze the symmetries of the hexatangle and give a list of Artin $n$-presentations for the trivial group. These presentations correspond to the double-branched covers of the hexatangle that produce $S^3$ after Dehn surgery. Also, using a result of Birman and Menasco (1994), we determine which closed pure $3$-braids are hyperbolic.

==> figures/table_factorized.tex <==
\begin{displaymath} \label{tabla1.2}
 \begin{array}{|r|c|c|c|}
 \hline

 %& r_1 & r_2 & r_3 &  \\
 \textrm{No.}& r_1
 &  r_2
 &   r_3\\
 &&&\\
 \hline
 \hline

 \hline
  1 &x_2x_3x_2x_1^{-1} &x_1^2(x_1x_3x_2^{-1}x_3^{-1})^{-\beta}x_3x_2x_1^{-1} &x_2^2x_3x_2(x_1x_3x_2^{-1}x_3^{-1})^{-\beta}x_3x_2x_1^{-1}\\

 \hline
  2 &x_3^{-2}(x_2x_3)^{-\beta}x_1x_2x_3 &x_1^{-1}(x_2x_3)^{-\beta}x_2^{-1}(x_2x_3)^{\beta}x_2x_3 &x_2^2(x_2x_3)^{-2\beta}x_2^{-1}(x_2x_3)^{\beta}x_2x_3\\

 \hline
  3 &x_3^{-2}x_2^{-1}x_1x_2x_3 &x_1^{-2}(x_1x_3^{-1}x_2x_3)^{-\beta}x_1x_2x_3 &x_2^2x_3^{-1}x_2^{-1}(x_1x_3^{-1}x_2x_3)^{-\beta}x_1x_2x_3\\

 \hline
  4 &x_2^{-2}x_3x_1x_3^{-1}x_2 &(x_1)^{-\beta}x_2^{-1}x_3x_2x_1^{-1}x_2^{-1}x_3x_2x_3^{-1}x_2 &x_3^{-2}(x_2^{-1}x_3)^2x_2x_1^{-1}x_2^{-1}x_3x_2x_3^{-1}x_2\\

 \hline
  5 &x_1^2(x_3^{-1}x_1)^{-\beta}x_1^{-1}x_3x_2 &x_2^{-1}(x_3^{-1}x_1)^{-\beta}x_3(x_3^{-1}x_1)^{\beta}x_2x_1^{-1}x_3x_2 &x_3^2(x_3^{-1}x_1)^{-2\beta}x_3(x_3^{-1}x_1)^{\beta}x_2x_1^{-1}x_3x_2\\

 \hline
  6 &x_2x_3x_2x_1 &x_1^{-2}(x_3x_2x_3^{-1}x_1)^2x_3x_2x_1 &(x_2^{-1})^{-\beta}(x_3x_2)^2x_3^{-1}x_1x_3x_2x_3^{-1}x_1x_3x_2x_1\\

 \hline
  7 &x_2x_3(x_1x_3^{-1}x_2)^{-\beta} &x_1(x_2^{-1}x_3x_2x_1^{-1})^2(x_1x_3^{-1}x_2)^{-\beta} &(x_3x_2^{-1})^2x_3x_2x_1^{-1}x_2^{-1}x_3x_2x_1^{-1}(x_1x_3^{-1}x_2)^{-\beta}\\

 \hline
  8 &x_3^{-1}x_2(x_3x_2x_1)^2 &x_1^{-1}(x_1^{-1}x_3x_2^{-1}x_3^{-1})^{-\beta}(x_3x_2x_1)^2 &x_2x_3x_2(x_1^{-1}x_3x_2^{-1}x_3^{-1})^{-\beta}(x_3x_2x_1)^2\\

 \hline
  9 &(x_2)^{-\beta}(x_2^{-1}x_3)^2x_1x_3^{-1}x_2 &x_1^{-1}(x_2^{-1}x_3)^2(x_2x_3^{-1})^2x_2 &x_3^{-2}(x_2^{-1}x_3)^4(x_2x_3^{-1})^2x_2\\

 \hline
  10 &(x_2)^{-\beta}x_1x_2x_3 &(x_1x_2)^2x_1(x_2^{-1}x_1^{-1})^3x_3 &x_1^{-1}x_2x_1x_2x_3^{-1}(x_1x_2)^2x_1(x_2^{-1}x_1^{-1})^3x_3\\

 \hline
  11 &x_3^{-1}(x_2x_3)^{-\beta}(x_1x_2x_3)^2 &x_1^{-2}(x_2x_3)^{-\beta}x_2^{-1}(x_2x_3)^{\beta}x_2x_3x_1x_2x_3 &x_2(x_2x_3)^{-2\beta}x_2^{-1}(x_2x_3)^{\beta}x_2x_3x_1x_2x_3\\

 \hline
  12 &x_3^{-3}x_2^{-1}(x_1x_2x_3)^2 &x_1^{-1}(x_1x_3^{-1}x_2x_3)^{-\beta}(x_1x_2x_3)^2 &x_2x_3^{-1}x_2^{-1}(x_1x_3^{-1}x_2x_3)^{-\beta}(x_1x_2x_3)^2\\

 \hline
  13 &x_3^2x_1x_3^{-1}x_2 &(x_1x_3^{-1})^2x_1(x_3x_1^{-1})^3x_2 &(x_1)^{-\beta}(x_1x_3^{-1})^2x_2^{-1}(x_1x_3^{-1})^2x_1(x_3x_1^{-1})^3x_2\\

 \hline
  14 &x_3^{-1}(x_2x_3)^2x_2x_1 &x_1^{-1}(x_3x_2)^2x_3^{-1}x_2^{-1}x_3^{-1}x_1x_3x_2x_1 &(x_2^{-1})^{-\beta}(x_3x_2)^4x_3^{-1}x_2^{-1}x_3^{-1}x_1x_3x_2x_1\\

 \hline
  15 &x_3x_2 &x_2x_1x_3^{-1}x_1x_3x_1^{-1}x_2^{-1}x_1x_3^{-1}x_1(x_3x_1^{-1})^2x_2 &(x_1)^{-\beta}x_1x_3^{-1}x_2^{-1}x_1x_3^{-1}x_1x_3x_1^{-1}x_2^{-1}x_1x_3^{-1}x_1(x_3x_1^{-1})^2x_2\\

 \hline
  16 &x_3x_1^{-1} &(x_1)^{-\beta}x_1x_2x_3^{-1}x_2x_3x_2^{-1}x_1x_2x_3^{-1}x_2(x_3x_2^{-1})^2x_1^{-1} &x_2^{-1}x_3^{-1}x_1x_2x_3^{-1}x_2x_3x_2^{-1}x_1x_2x_3^{-1}x_2(x_3x_2^{-1})^2x_1^{-1}\\

 \hline
  17 &x_3x_2^{-1}x_3(x_1x_3^{-1}x_2)^{-\beta} &x_1^2(x_2^{-1}x_3)^2x_2x_3^{-1}x_2x_1^{-1}(x_1x_3^{-1}x_2)^{-\beta} &(x_3x_2^{-1})^4x_3x_2x_3^{-1}x_2x_1^{-1}(x_1x_3^{-1}x_2)^{-\beta}\\

 \hline
  18 &x_3^{-1}(x_2x_3)^2(x_1x_2x_3)^{-\beta} &x_1^{-1}(x_2x_3)^2x_2(x_3^{-1}x_2^{-1})^2(x_1x_2x_3)^{-\beta} &x_3x_2x_3x_1(x_2x_3)^2x_2(x_3^{-1}x_2^{-1})^2(x_1x_2x_3)^{-\beta}\\

 \hline
  19 &(x_3)^{-\beta}x_3^{-1}x_2^{-1}(x_1x_2x_3)^2 &(x_1^{-1}x_3^{-1}x_2^{-1}x_3)^2x_2x_3x_1x_2x_3 &x_2(x_3^{-1}x_2^{-1})^2x_3x_1^{-1}x_3^{-1}x_2^{-1}x_3x_2x_3x_1x_2x_3\\

 \hline
  20 &x_3^{-2}x_2x_3(x_1x_2x_3)^{-\beta} &x_2x_3x_2x_3^{-1}x_2^{-1}x_1x_2x_3x_2x_3^{-1}x_2^{-1}(x_1x_2x_3)^{-\beta} &x_3(x_1x_2x_3x_2x_3^{-1}x_2^{-1})^2(x_1x_2x_3)^{-\beta}\\

 \hline
  21 &x_1(x_3^{-1}x_1)^{-\beta}(x_1^{-1}x_3x_2)^2 &x_2^{-2}(x_3^{-1}x_1)^{-\beta}x_3(x_3^{-1}x_1)^{\beta}(x_2x_1^{-1}x_3)^2x_2 &x_3(x_3^{-1}x_1)^{-2\beta}x_3(x_3^{-1}x_1)^{\beta}(x_2x_1^{-1}x_3)^2x_2\\

 \hline
  22 &x_3^{-2}x_2^{-1}x_3^{-1}x_2^{-1}(x_1x_2x_3)^2 &(x_1)^{-\beta}(x_3^{-1}x_2^{-1})^2(x_3x_2)^2x_3x_1x_2x_3 &x_2(x_3^{-1}x_2^{-1})^4(x_3x_2)^2x_3x_1x_2x_3\\

 \hline
  23 &(x_3^{-1})^{-\beta}x_1x_3x_2x_1 &x_2^{-1}x_3^{-1}x_2^{-1}x_3x_2x_1^{-1}x_2^{-1}x_3^{-1}x_2^{-1}(x_3x_2)^2x_1x_3x_2x_1 &x_3^{-1}x_1^{-1}x_2^{-1}x_3^{-1}x_2^{-1}x_3x_2x_1^{-1}x_2^{-1}x_3^{-1}x_2^{-1}(x_3x_2)^2x_1x_3x_2x_1\\

 \hline
  24 &x_3x_2^{-1}x_3^{-1}x_1x_3x_2x_1 &(x_1^{-1})^{-\beta}x_1^{-1}(x_2^{-1}x_3^{-1})^2x_2^{-1}(x_3x_2)^3x_1x_3x_2x_1 &x_3^{-1}x_2^{-1}x_3^{-1}x_1^{-1}(x_2^{-1}x_3^{-1})^2x_2^{-1}(x_3x_2)^3x_1x_3x_2x_1\\

\hline
 \end{array}
\end{displaymath}


